Webcam-based Eye Gaze Tracking under Natural Head Movement

This manuscript investigates and proposes a visual gaze tracker that tackles the problem using only an ordinary web camera and no prior knowledge in any sense (scene set-up, camera intrinsic and/or extrinsic parameters). The tracker we propose is based on the observation that our desire to grant the freedom of natural head movement to the user requires 3D modeling of the scene set-up. Although, using a single low resolution web camera bounds us in dimensions (no depth can be recovered), we propose ways to cope with this drawback and model the scene in front of the user. We tackle this three-dimensional problem by realizing that it can be viewed as series of two-dimensional special cases. Then, we propose a procedure that treats each movement of the user's head as a special two-dimensional case, hence reducing the complexity of the problem back to two dimensions. Furthermore, the proposed tracker is calibration free and discards this tedious part of all previously mentioned trackers. Experimental results show that the proposed tracker achieves good results, given the restrictions on it. We can report that the tracker commits a mean error of (56.95, 70.82) pixels in x and y direction, respectively, when the user's head is as static as possible (no chin-rests are used). Furthermore, we can report that the proposed tracker commits a mean error of (87.18, 103.86) pixels in x and y direction, respectively, under natural head movement.

==> Solution.tex <==
\chapter{Proposed Solution}\label{chapter:solution}

\dropping{2}{H}\newline aving defined the problem, let's introduce our direct answer to the challenge described in section \ref{sec:problem}. In this chapter we present and discuss the proposed solution in details. The proposed solution tackles the problem directly, first in two dimensions and then in three dimensions so, there are two different systems implemented for this project. The static visual gaze tracker (2D) discussed in section \ref{sec:2D} is implemented as a proof of concept. It is entirely 2D in sense that, it uses no information regarding the position of the head in 3D space. The main contribution of this system is that it proves that highly accurate tracking of the visual gaze, when using a single low resolution web camera, is possible with the restriction that the subject's head must be as static as possible. The dynamic tracker (3D) discussed in section \ref{sec:3D} on the other hand, is the proposed solution of the problem when the subject is granted with the freedom of natural head movement. The dynamic tracker itself is offering two different algorithms that, will turn to be suitable for different situations - in the text the first one is regarded as 2.5D and it is suitable when the subject's head does not move too much, while the second (3D) is suitable when the subject's head performs large movements.

Figure \ref{fig:eyeTrackingTechniques} gives the general overview of eye tracking techniques in the literature. In order to comply with the usability requirements discussed earlier (section \ref{sec:problem}) we had built a system that can be classified as a non-intrusive, 3D+2D, and appearance based. Huge amount of research has been done on possible solutions of this problem, and it seems that there is no algorithm similar to the proposed solution. The short description of the proposed solution would be that, the knowledge for the position of the head in 3D space, which defines the overall visual gaze direction, can be exploited through the simplicity of the 2D approach.

\section{Static Tracker (2D)}\label{sec:2D}

In this section we present our first attempt to cope with the problem at hand. At this end, it is clear that highly accurate tracking of the visual gaze on the computer screen with the restriction of a static head, is possible through simple and efficient computer vision algorithms.

Our approach to this is non-intrusive, 2D, and appearance based. However, it is not based on PCCR (Pupil-Center-Corneal Reflection), but solely on image analysis. Generally, the system is composed of four steps (two steps in each of the components of the the visual gaze estimation pipeline - Figure \ref{fig:gazePipeline}). In the first component we need a method to detect and track the location of the eyes, and a method to define and track facial features. In the second component, a calibration procedure is performed that, gives us correspondences between facial feature-pupil center vectors and the computer screen coordinates, and a method to find a solution for future visual gaze estimation. In our case, the method of least squares (Appendix \ref{chapter:AppendixB}) is applied to approximate solution of overdetermined system of equations.

\subsection{Tracking the Eyes}\label{subsec:eyes}

Since we assume that the user's head is static in this scenario, it is evident that, the accurate detection and tracking of the location of the eyes is at most importance for the performance of the 2D visual gaze tracker. Our first attempt for eye location estimation and tracking is based on the template matching technique. Template matching is a technique in digital image processing for finding small parts of an image which match a template image.

This method is normally implemented by first picking out a part of the search image to use as a template. Template matching matches an actual image patch against an input image by `sliding' the patch over the input image using a matching method. For example, if, we have an image patch containing a face then, we can slide that face over an input image looking for strong matches that would indicate that another face is present. Let's use $I$ to donate the input image (where we are searching), $T$ the template, and $R$ the result. Then, 
\begin{itemize}
\item{\textbf{squared difference} matching method matches the squared difference, so a perfect match will be 0 and bad match will be large:}
\begin{equation}
R_{sq\_diff}(x,y) = \displaystyle\sum_{x',y'}[T(x',y') - I(x + x',y + y')]^{2}
\end{equation}
\item{\textbf{correlation} matching method multiplicatively matches the template against the image, so a perfect match will be large and bad match will be small or 0:}
\begin{equation}
R_{ccorr}(x,y) = \displaystyle\sum_{x',y'}[T(x',y')\cdot I(x + x',y + y')]^{2}
\end{equation}
\item{\textbf{correlation coefficient} matching method matches a template relative to its mean against the image relative to its mean, so a perfect match will be 1 and a perfect mismatch will be -1; a value of 0 simply means that there is no correlation (random alignments):}
\begin{equation}
R_{ccoeff}(x,y) = \displaystyle\sum_{x',y'}[T'(x',y')\cdot I'(x + x',y + y')]^{2}
\end{equation}
\begin{equation}
T'(x',y') = T(x',y') - \frac{1}{(w\cdot h)\displaystyle\sum_{x'',y''}T(x'',y'')}
\end{equation}
\begin{equation}
I'(x + x',y + y') = I(x + x',y + y') - \frac{1}{(w\cdot h)\displaystyle\sum_{x'',y''}I(x + x'',y + y'')}
\end{equation}
\item{\textbf{normalized methods} - for each of the three methods just described, there are also normalized versions first developed by Galton \cite{GALTON} as described by Rodgers \cite{RODGERS&NICEWANDER}. The normalized methods are useful because, they can help to reduce the effects of lighting differences between the template and the image. In each case, the normalization coefficient is the same:}
\begin{equation}
Z(x,y) = \sqrt{\displaystyle\sum_{x',y'}T(x',y')^{2}\cdot \displaystyle\sum_{x',y'}I(x + x',y + y')^{2}}
\end{equation}
The values for method that give the normalized computations are:
\begin{equation}
R_{sq\_diff\_normed}(x,y) = \frac{R_{sq\_diff}(x,y)}{Z(x,y)}
\end{equation}
\begin{equation}
R_{ccor\_normed}(x,y) = \frac{R_{ccor}(x,y)}{Z(x,y)}
\end{equation}
\begin{equation}
R_{ccoeff\_normed}(x,y) = \frac{R_{ccoeff}(x,y)}{Z(x,y)}
\end{equation}
\end{itemize}

Template matching has the advantage to be very intuitive and easy to implement. Unfortunately, there are important drawbacks associated with it: first, the template needs to be selected by hand every time the system is used, and second, the accuracy of the technique is generally not very high. Furthermore, the accuracy is highly dependent on the lightening conditions: if the lightening conditions are too different between the template and the search image then, it results in very poor accuracy for the estimate of the location of the eye.

Figure \ref{fig:templateMatching} illustrates the procedure of template matching based on squared difference matching method: left eye template (a), right eye template (b), and their matches in the search image (c). The eye regions are selected at the beginning of the procedure and then, the regions with high response to the templates are found in the search image.

\begin{figure}[htpd!]
\begin{center}
\subfigure[]{
\includegraphics[scale=1]{./images/png/leftTemplate.png}}
\subfigure[]{
\includegraphics[scale=1]{./images/png/rightTemplate.png}}
\subfigure[]{
\includegraphics[scale=0.25]{./images/png/templateTracking.png}}
\caption{Template matching}
\label{fig:templateMatching}
\end{center}
\end{figure}

Considering this drawbacks, we decided to use another technique for accurate eye center location estimation and tracking. This technique is based on image isophotes (areas of equal intensity in the image). A full discussion of this algorithm is outside the scope of this text, but the basic procedure is described next. For a full discussion, we refer the reader to \cite{VALENTI&GEVERS}.

The isophotes of an image are curves connecting points of equal intensity. Since isophotes do not intersect each other, an image can be fully described by its isophotes. Furthermore, the shape of the isophotes is independent to rotation and linear lighting changes. Due to these properties, isophotes have been successfully used as features in object detection and image segmentation. To better illustrate the well known isophote framework, we introduce the notion of intrinsic geometry, i.e. geometry with a locally defined coordinate system. In every point of the image, a local coordinate frame is fixed in such a way that it points in the direction of the maximal change of the intensity, which corresponds to the direction of the gradient. This reference frame $\{v, w\}$ is referred to as the \textit{gauge coordinates}. Its frame vectors $\hat{w}$ and $\hat{v}$ are defined as:

\begin{equation}
\hat{w} = \frac{\{L_{x},L_{y}\}}{\sqrt{L_{x}^{2}+L_{y}^{2}}}; \hat{v} = \perp\hat{w}
\end{equation}
where $L_{x}$ and $L_{y}$ are the first-order derivatives of the luminance function $L(x,y)$ in the $x$ and $y$ dimension, respectively. In this setting, a derivative in the $w$ direction is the gradient itself, and the derivative in the $v$ direction (perpendicular to the gradient) is 0 (no intensity change along the isophote).

In this coordinate system, an isophote is defined as $L(v,w(v)) = constant$ and its curvature is defined as the change $w''$ of the tangent vector $w'$. By implicit differentiation with respect to $v$ of the isophote definition, we have:

\begin{equation}
L_{v} + L_{w}w' = 0; w' = -\frac{L_{v}}{L_{w}}
\end{equation}

Since we know from the gauge condition that $L_{v} = 0$, we have $w' = 0$. Differentiating again with respect to $v$, yields:

\begin{equation}
L_{vv} + 2L_{vv}w' + L_{ww}w'^{2} + L_{w}w'' = 0
\end{equation}

Solving for $\kappa = w''$ (the isophote curvature) and knowing that $w' = 0$, the isophote curvature is obtained as:

\begin{equation}
\kappa = -\frac{L_{vv}}{L_{w}}
\end{equation}

In Cartesian coordinates, this becomes \cite{DAM&ROMENY}, \cite{GINKEL&WEIJER&VLIET&VERBEEK}:

\begin{equation}\label{eq:kappa}
\kappa = -\frac{L_{vv}}{L_{w}} = -\frac{L_{y}^{2}L_{xx} - 2L_{x}L_{xy}L_{y} + L_{x}^{2}L_{yy}}{(L_{x}^{2} + L_{y}^{2})^\frac{3}{2}}
\end{equation}

Since the curvature is the reciprocal of the radius, we can reverse equation (\ref{eq:kappa}) to obtain the radius of the circle that generated the curvature of the isophote. The radius is meaningless if it is not combined with orientation and direction. The orientation can be estimated from the gradient but its direction will always point towards the highest change in the luminance. However, the sign of the isophote curvature depends on the intensity of the outer side of the curve (for a brighter outer side the sign is positive). Thus, by multiplying the gradient with the inverse of the isophote curvature, the duality of the isophote curvature helps in disambiguating the direction of the center. Since the gradient can be written as $\frac{\{L_{x},L_{y}\}}{L_{w}}$, we have:

\begin{eqnarray}
D(x,y) & = & \frac{\{L_{x},L_{y}\}}{L_{w}}\left(-\frac{L_{w}}{L_{vv}}\right)\\
& = & -\frac{\{L_{x},L_{y}\}}{L_{vv}}\\
& = & -\frac{\{L_{x},L_{y}\}(L_{x}^{2} + L_{y}^{2})}{L_{y}^{2}L_{xx} - 2L_{x}LL_{xy}L_{y} + L_{x}^{2}L_{yy}}
\end{eqnarray}
where $D(x,y)$ are the displacement vectors to the estimated position of the centers, which can be mapped into an accumulator. Since every vector gives a rough estimate of the center, we can convolve the accumulator with a Gaussian kernel so that each cluster of votes will form a single center estimate. The contribution of each vector can be weighted according to a relevance mechanism.

The main idea is that by collecting and averaging local evidence of curvature, the discretization problems in a digital image could be lessened and accurate center estimation could be achieved. The curvedness, indicating how curved a shape is, was introduced as:

\begin{equation}
curvedness = \sqrt{L_{xx}^{2} + 2L_{xy}^{2} + L_{yy}^{2}}
\end{equation}

We note that the curvedness has low response on flat surfaces and edges, whereas it yields high response in places where the isophote density is maximal. As observed before, the isophote density is maximal around the
edges of an object, meaning that by selecting the parts of the isophotes where the curvedness is maximal, they will likely follow an object boundary and locally agree on the same center. It is clear that the curvedness is higher where the isophotes are equally distributed. The advantage of the proposed approach over a pure edge based method is that, by using the curvedness as the voting scheme for the importance of the vote, every pixel in the image may contribute to a decision. By summing the votes, we obtain high response on isocentric isophotes patterns which respect the constraint of being near edges.

Recalling that the sign of the isophote curvature depends on the intensity of the outer side of the curve, we observe that a negative sign indicates a change in the direction of the gradient (i.e. from brighter to darker areas). Therefore, it is possible to discriminate between dark and bright centers by analyzing the sign of the curvature. Regarding the specific task of cornea and iris location, it can be assumed that the sclera is brighter than the cornea and the iris, so we should ignore the votes in which the curvature is positive, that is, where it agrees with the direction of the gradient.

Mean shift usually operates on back-projected images in which probabilities are assigned to pixels based on the color probability distribution of a target, weighted by a spatial kernel over pixel locations. It then finds the local maximum of this distribution by gradient ascent. Here, the mean shift procedure is directly applied to the centermap resulting from our method, under the assumption that the most relevant center should have higher density of votes, and that wrong centers are not so distant from the correct one (e.g. on an eye corner). A mean shift search window is initialized on the centermap, centered on the found center. The algorithm then iterates to converge to a region with maximal distribution. After some iteration, the center closest to the center of the search window is selected as the new eye center estimate.

\subsection{Tracking the Features}\label{subsec:features}

Since the second component of the visual gaze estimation pipeline uses both the information for the location of the facial features and the location of the eyes it is crucial that the features are tracked with highest accuracy possible. In this early system we implemented very simple approach for facial feature tracking based on Lucas-Kanade method for optical flow estimation. The feature is selected in the first frame and then its location is tracked. A full discussion of this algorithm is outside the scope of the text, but the basic procedure is described next. For a full discussion, we refer the reader to \cite{LUCAS&KANADE}.

The translational image registration problem can be characterized as follows: we are given functions $F(x)$ and $G(x)$ which give the respective pixel values at each location $x$ in two images. We wish to find the disparity vector $h$ that minimizes some measure of difference between $F(x + h)$ and $G(x)$, for $x$ in some region of interest $R$.

Typical measures of the difference between $F(x + h)$ and $G(x)$ are:
\begin{itemize}
\item{\textbf{$\mathbf{L}_{1}$ norm}}
\begin{equation}
\displaystyle\sum_{x \in R}[F(x + h) - G(x)]
\end{equation}
\item{\textbf{$\mathbf{L}_{2}$ norm}}
\begin{equation}
\left( \displaystyle\sum_{x \in R}[F(x + h) - G(x)]^{2}\right)^{\frac{1}{2}}
\end{equation}
\item{\textbf{negative of normalized correlation}}
\begin{equation}
\frac{- \displaystyle\sum_{x \in R}F(x + h)G(x)}{\left( \displaystyle\sum_{x \in R}F(x + h)^{2}\right)^{\frac{1}{2}}\left( \displaystyle\sum_{x \in R}G(x)^{2}\right)^{\frac{1}{2}}}
\end{equation}
\end{itemize}
In the one-dimensional registration problem, we wish to find the horizontal disparity $h$ between two curves $F(x)$ and $G(x) = F(x + h)$. This is illustrated in Figure \ref{fig:disparity}.

\begin{figure}[htpd!]
\begin{center}
\includegraphics[scale=0.5]{./images/pdf/lucasKanade.pdf}
\caption{One-dimensional registration problem}
\label{fig:disparity}
\end{center}
\end{figure}
The solution to this problem depends on a linear approximation to the behavior of $F(x)$ in the neighborhood of $x$. In particular, for small $h$,
\begin{equation}\label{eq:disparity1}
F'(x) \approx \frac{F(x + h) - F(x)}{h} = \frac{G(x) - F(x)}{h}
\end{equation}
so that,
\begin{equation}\label{eq:disparity2}
h \approx \frac{G(x) - F(x)}{F'(x)}
\end{equation}
The success of the algorithm requires $h$ to be small enough that this approximation is adequate.

The approximation to $h$ given in (\ref{eq:disparity2}) depends on $x$. A natural method for combining the various estimates of $h$ at various values of $x$ would be simply to average them:
\begin{equation}\label{eq:disparity3}
h \approx \frac{\displaystyle\sum_{x}\frac{G(x) - F(x)}{F'(x)}}{\displaystyle\sum_{x}1}
\end{equation}

We can improve this average by realizing that the linear approximation in (\ref{eq:disparity1}) is good where $F(x)$ is nearly linear, and conversely is worse where $|F''(x)|$ is large. Thus, we could weight the contribution of each term to the average in (\ref{eq:disparity3}) in inverse proportion to an estimate of $|F''(x)|$. One such estimate is
\begin{equation}\label{eq:disparity4}
F''(x) \approx \frac{G'(x) - F'(x)}{h}
\end{equation}

Since our estimate is to be used as a weight in an average, we can drop the constant factor of $\frac{1}{h}$ in (\ref{eq:disparity4}), and use as our weighting function
\begin{equation}\label{eq:disparity5}
w(x) = \frac{1}{|G'(x) - F'(x)|}
\end{equation}

This appeals to our intuition; for example, in Figure \ref{fig:disparity}, where the two curves cross, the estimate of $h$ provided by (\ref{eq:disparity2}) is 0, which is bad; fortunately, the weight given to this estimate in the average is small, since the difference between $F'(x)$ and $G'(x)$ at this point is large. The average with weighting is
\begin{equation}\label{eq:disparity6}
h = \frac{\displaystyle\sum_{x}\frac{w(x)[G(x) - F(x)]}{F'(x)}}{\displaystyle\sum_{x}w(x)}
\end{equation}
where $w(x)$ is given by (\ref{eq:disparity5}).

Having obtained this estimate, we can move $F(x)$ by our estimate of $h$, and repeat this procedure, yielding a type of Newton-Raphson iteration. Ideally, our sequence of estimates of $h$ will converge to the best $h$. This iteration is expressed by
\begin{equation}\label{eq:disparity7}
\begin{array}{l}
h_{0} = 0, \\
h_{k + 1} = h_{k} + \frac{\displaystyle\sum_{x}\frac{w(x)[G(x) - F(x)]}{F'(x)}}{\displaystyle\sum_{x}w(x)}
\end{array}
\end{equation}

The derivation given above does not generalize well to two dimensions because the two-dimensional linear approximation occurs in a different form. Moreover, (\ref{eq:disparity2}) is undefined where $F'(x) = 0$, i.e. where the curve is level. Both of these problems can be corrected by using the linear approximation of equation (\ref{eq:disparity1}) in the form
\begin{equation}\label{eq:disparity8}
F(x + h) \approx F(x) + hF'(x)
\end{equation}
to find the $h$ that minimizes the $\mathbf{L}_{2}$ norm measure of difference between the curves:
\begin{equation*}
E = \displaystyle\sum_{x}[F(x + h) - G(x)]^{2}
\end{equation*}
To minimize the error with respect to $h$, we set
\begin{eqnarray*}
0 & = & \frac{\partial E}{\partial h} \\
& \approx & \frac{\partial}{\partial h}\displaystyle\sum_{x}[F(x) + hF'(x) - G(x)]^{2} \\
& = & \displaystyle\sum_{x}2F'(x)[F(x) + hF'(x) - G(x)]
\end{eqnarray*}
from which
\begin{equation}\label{eq:disparity9}
h \approx \frac{\displaystyle\sum_{x}F'(x)[G(x) - F(x)]}{\displaystyle\sum_{x}F'(x)^{2}}
\end{equation}

This is essentially the same solution that is derived in (\ref{eq:disparity6}), but with the weighting function $w(x) = F'(x)^{2}$. This form of linear approximation generalizes to two or more dimensions \cite{LUCAS&KANADE}. Moreover, we have avoided the problem of dividing by 0, since (\ref{eq:disparity9}) we will divide by 0 only if $F'(x) = 0$ \textit{everywhere} (in which case $h$ really is undefined), whereas in (\ref{eq:disparity3}) we will divide by 0 if $F'(x) = 0$ \textit{anywhere}.

The iterative form with weighting corresponding to (\ref{eq:disparity7}) is
\begin{equation}\label{eq:disparity10}
\begin{array}{l}
h_{0} = 0, \\
h_{k + 1} = h_{k} + \frac{\displaystyle\sum_{x}w(x)F'(x + h_{k})[G(x) - F(x + h_{k})]}{\displaystyle\sum_{x}w(x)F'(x + h_{k})^{2}}
\end{array}
\end{equation}
where $w(x)$ is given by (\ref{eq:disparity5}).

In our case, we use the algorithm to obtain the coordinates of the facial features in some frame $a$, given the coordinates of the facial features in an earlier frame $b$, along with the image data of frames $a$ and $b$, allowing the tracking of the facial features.

\subsection{Calibration Techniques}\label{subsec:calibration}

The precise mapping from facial feature-pupil center vectors to screen coordinates is necessary for accurate visual gaze tracking system. This mapping is achieved through a calibration procedure. During the calibration step, correspondences between the facial feature-pupil center vectors and screen coordinates are obtained. The calibration procedure is done using a set of 25 points distributed evenly on the computer screen (Figure \ref{fig:calibrationTechniques}). The subject is asked to draw a point as near as possible to the position in the template image using the mouse. As the reader can guess, it is inevitable to introduce errors in the system at this stage.

Consider the following scenario: you sitting in front of the computer screen and been asked to gaze at a certain point on it. We can argue that even a human is not capable of telling in pixel coordinates precision the coordinates of the point that he/she is looking at. Indeed, a region around that point is the best we can get. Further discussion on this observation is offered later in the text (section \ref{sec:experimentsConclusions}) - the physiological limitations imposed by the structure of the human eye and the process of visual perception in human beings. For these reasons, we chose this type of calibration procedure; by tracking the mouse cursor movement with the eyes and clicking at the desire position, we ensure to record as close as possible, the eye saccade that is paired with the point on the screen under consideration. Furthermore, there is research done on the choice of the cursor shape for calibration purposes. It shows that the cursor's shape has an impact on the precision with which a human looks at it. We will not dive too deep in this discussion because our goal is to build a calibration free system where these observations and choices will not play a significant role. Once the subject clicks on the screen a recording is done for both eyes simultaneously.

\begin{figure}[htpd!]
\begin{center}
\includegraphics[scale=0.65]{./images/pdf/calibrationTechniques.pdf}
\caption{Calibration template}
\label{fig:calibrationTechniques}
\end{center}
\end{figure}

After the calibration procedure finishes, several models for solution estimation are used: 2D mapping with interpolation model that uses 2 points (21 and 5 or 1 and 25), linear model that uses 5 points (21, 25, 13, 1 and 5), and second order model that uses 9 or 25 points (21, 23, 25, 11, 13, 15, 1, 3 and 5 or all). The details of the model selection and the mathematics behind are given in section \ref{sec:solution}.

\section{Dynamic Tracker (3D)}\label{sec:3D}

This section presents an idea of how to incorporate our knowledge for the 3D position of the user's head into the 2D system discussed till now. This will grant the freedom of natural head movement to the user, while still exploits the simplicity of the entirely 2D approach.

Up till now, the point of visual gaze is estimated only according to the facial feature-pupil center vectors, which means that, the system is static, the accuracy is related to the position of the user's head. The more the user's head position differs from the position at which the calibration is done the poorer the accuracy of the estimated point of visual gaze. To overcome this limitations we have the following idea.

Figure \ref{fig:scenario3D1} illustrates the scene setup (same as discussed till now) in 3D space. We are using a cylindrical 3D head pose tracker algorithm based on Lukas-Kanade optical flow method \cite{XIAO&KANADE&COHN}. The depth of the user's head, that is the distance of the user's head to the computer screen (zero plane), is assumed to be initialized at $750mm$ from the camera origin \textit{(camera plane == screen plane?)}.

\begin{figure}[htpd!]
\begin{center}
\includegraphics[scale=0.75]{./images/pdf/scenario3D1.pdf}
\caption{The scene setup in 3D}
\label{fig:scenario3D1}
\end{center}
\end{figure}

Our idea is to define an \textit{user plane} in 3D space that is attached to the user's head. Since during the calibration procedure we obtain facial feature-pupil center vectors and the corresponding screen coordinates, our idea is to populate the constructed user plane with the obtained calibration points. More specifically, we trace a ray starting at the user's head origin (cylinder's origin) to the calibration point on the computer screen (zero plane). Then, we calculate the intersection point of that ray with the user plane. This procedure is repeated for each calibration point, so a set of \textit{user points} is defined at the beginning and that set is used to correct the calibration when the user moves his/her head. We refer the reader to Appendix \ref{chapter:appendixC} for detailed discussion on the mathematics behind line-plane intersection in 3D space. Figure \ref{fig:scenario3D2} illustrates the idea.

\begin{figure}[htpd!]
\begin{center}
\includegraphics[scale=0.65]{./images/pdf/scenario3D2.pdf}
\caption{User plane and user points}
\label{fig:scenario3D2}
\end{center}
\end{figure}

Due to the properties of the user plane - it is attached to the user's head when, the user moves his/her head the intersections with the zero plane will change. At this point, we can trace a ray starting at an user point to the user's head origin (cylinder's origin). Then, we calculate the intersection point of that ray with the zero plane. If we repeat this procedure for each user point, a set of new calibration points on the computer screen can be constructed each time the user moves his/her head. Having the new set of calibration points, we can solve again for the point of visual gaze. In this way we incorporate 3D information for the position of the user's head while still exploiting the simplicity of the 2D solution. Figure \ref{fig:scenario3D3} illustrates a movement of the user's head and the new intersection points (calibration points) used for re-calibration.

\begin{figure}[htpd!]
\begin{center}
\includegraphics[scale=0.65]{./images/pdf/scenario3D3.pdf}
\caption{New intersection points for re-calibration}
\label{fig:scenario3D3}
\end{center}
\end{figure}

In this new system we use the eye tracker described in \cite{VALENTI&GEVERS}. For the facial feature location we use the location of the origin of the user's head (origin of the cylindrical model), so we do not need to define it manually anymore. The facial feature-pupil center vectors are obtained in pose normalized coordinates which we could exploit. Namely, since we require an initialization at $750mm$ from the camera origin, a set of pose normalized facial feature-pupil center vectors can be obtained and used for future calibrations. This can be achieved by asking the user to start the system once he/she is in certain position relative to the computer screen using visual queues on the screen. This ensures that we can use the pre-obtained facial feature-pupil center vectors and the pre-defined calibration points on the computer screen. This in turn leads to calibration free system.

\section{Solution}\label{sec:solution}

The problem we are facing is computing the point of gaze in screen coordinates given the current facial feature-pupil center vector in camera coordinates. The facial feature-pupil center vector is constructed upon the current location of the eye and the location of the facial feature. We can view this problem, as like there is an unknown function that maps our input (facial feature-pupil center vector) to specific output (point on the computer screen). Furthermore, this problem can be viewed as a simple regression problem, namely, suppose we observe a real-valued input variable $\mathnormal{x}$ (facial feature-pupil center vector) and we wish to use this observation to predict the value of a real-valued target variable $\mathnormal{t}$ (point on the computer screen). We would like to learn the model (function) that is able to generate the desired output given the input.

Suppose we are given a training set (constructed during the calibration step) comprising $\mathnormal{N}$ observations of $\mathnormal{x}$, together with the corresponding observations of the values of $\mathnormal{t}$. Our goal is to exploit the training set in order to make predictions of the value $\mathnormal{\Hat{t}}$ of the target variable for some new value $\mathnormal{\Hat{x}}$ of the input variable. If we consider a simple approach based on curve fitting then we want to fit the data using a polynomial function of the form

\begin{equation}
y(x,\mathbf{w}) = w_{0} + w_{1}x + w_{2}x^{2} + ... + w_{M}x^{M} = \displaystyle\sum_{j=0}^{M}w_{j}x^{j}
\end{equation}
where $\mathnormal{M}$ is the order of the polynomial.

The values of the coefficients will be determined by fitting the polynomial to the training data. This can be done by minimizing an error function that measures the misfit between the function $\mathnormal{y(x,\mathbf{w})}$, for any given value of $\mathbf{w}$, and the training set data points. One simple choice of error function, which is widely used, is given by the sum of the squares of the errors between the predictions $\mathnormal{y(x_{n},\mathbf{w})}$ for each data point $\mathnormal{x_{n}}$ and the corresponding target values $\mathnormal{t_{n}}$, so that we minimize

\begin{equation}
E(\mathbf{w}) = \frac{1}{2}\displaystyle\sum_{n=1}^{N}\{y(x_{n},\mathbf{w}) - t_{n}\}^{2}
\end{equation}

The error function is a nonnegative quantity that would be zero if, and only if, the function $\mathnormal{y(x,\mathbf{w})}$ were to pass exactly through each training data point. We can solve the curve fitting problem by choosing the value of $\mathbf{w}$ for which $\mathnormal{E(\mathbf{w})}$ is as small as possible.

There remains the problem of choosing the order $\mathnormal{M}$ of the polynomial or so-called model selection. The models chosen for fitting our data are discussed next,

\begin{itemize}\label{list:models}
\item{\textbf{2D mapping with interpolation model} takes into account 2 calibration points (Figure \ref{fig:calibrationTechniques}, points: 21 and 5 or 1 and 25). The solution is computed using linear interpolation as follows:
\begin{eqnarray}
\mathnormal{s_{x}} = \mathnormal{s_{x1} + \frac{x - x_{1}}{x_{2} - x_{1}}(s_{x2} - s_{x1})} \nonumber \\
\mathnormal{s_{y}} = \mathnormal{s_{y1} + \frac{y - y_{1}}{y_{2} - y_{1}}(s_{y2} - s_{y1})}
\end{eqnarray}
For example, suppose the screen coordinates and the facial feature-pupil center vectors used for calibration in points P1 and P2 are respectively ($\mathnormal{s_{x1}}$, $\mathnormal{s_{y1}}$), ($\mathnormal{x_{1}}$, $\mathnormal{y_{1}}$) and ($\mathnormal{s_{x2}}$, $\mathnormal{s_{y2}}$), ($\mathnormal{x_{2}}$, $\mathnormal{y_{2}}$). Then after the measurement of the current facial feature-pupil center vector ($\mathnormal{x}$, $\mathnormal{y}$) is taken, the screen coordinates is computed using the above equations.}
\item{\textbf{linear model} takes into account 5 calibration points (Figure \ref{fig:calibrationTechniques}, points: 1, 5, 13, 21, 25). The mapping between facial feature-pupil center vectors and screen coordinates is done using the following equations:
\begin{eqnarray}
\mathnormal{s_{x}} = \mathnormal{a_{0} + a_{1}x} \nonumber \\
\mathnormal{s_{y}} = \mathnormal{b_{0} + b_{1}y}
\end{eqnarray}
where ($\mathnormal{s_{x}}$, $\mathnormal{s_{y}}$) are screen coordinates and ($\mathnormal{x}$, $\mathnormal{y}$) is the facial feature-pupil center vector. The coefficients $\mathnormal{a_{0}}$, $\mathnormal{a_{1}}$ and $\mathnormal{b_{0}}$, $\mathnormal{b_{1}}$ are the unknowns and can be found using least squares approximation (Appendix \ref{chapter:AppendixB}).}
\item{\textbf{second order model} takes into account a set of 9 (Figure \ref{fig:calibrationTechniques}, points: 1, 3, 5, 11, 13, 15, 21, 25, 23) or a set 25 (Figure \ref{fig:calibrationTechniques}, all points) calibration points. The mapping between facial feature-pupil center vectors and screen coordinates is done using the following equations:
\begin{eqnarray}
\mathnormal{s_{x}} = \mathnormal{a_{0} + a_{1}x + a_{2}y + a_{3}xy + a_{4}x^{2} + a_{5}y^{2}} \nonumber \\
\mathnormal{s_{y}} = \mathnormal{b_{0} + b_{1}x + b_{2}y + b_{3}xy + b_{4}x^{2} + b_{5}y^{2}}
\end{eqnarray}
where ($\mathnormal{s_{x}}$, $\mathnormal{s_{y}}$) are screen coordinates and ($\mathnormal{x}$, $\mathnormal{y}$) is the facial feature-pupil center vector. The coefficients $\mathnormal{a_{0}}, \mathnormal{a_{1}}, \mathnormal{a_{2}}, \mathnormal{a_{3}}, \mathnormal{a_{4}}, \mathnormal{a_{5}}$ and $\mathnormal{b_{0}}, \mathnormal{b_{1}}, \mathnormal{b_{2}}, \mathnormal{b_{3}}, \mathnormal{b_{4}}, \mathnormal{b_{5}}$ are the unknowns and can be found using least squares approximation (Appendix \ref{chapter:AppendixB}).}
\end{itemize}
\cleardoublepage

